Does a Face Mask Protect my Privacy?: Deep Learning to Predict Protected Attributes from Masked Face Images

Contactless and efficient systems are implemented rapidly to advocate preventive methods in the fight against the COVID-19 pandemic. Despite the positive benefits of such systems, there is potential for exploitation by invading user privacy. In this work, we analyse the privacy invasiveness of face biometric systems by predicting privacy-sensitive soft-biometrics using masked face images. We train and apply a CNN based on the ResNet-50 architecture with 20,003 synthetic masked images and measure the privacy invasiveness. Despite the popular belief of the privacy benefits of wearing a mask among people, we show that there is no significant difference to privacy invasiveness when a mask is worn. In our experiments we were able to accurately predict sex (94.7%),race (83.1%) and age (MAE 6.21 and RMSE 8.33) from masked face images. Our proposed approach can serve as a baseline utility to evaluate the privacy-invasiveness of artificial intelligence systems that make use of privacy-sensitive information. We open-source all contributions for re-producibility and broader use by the research community.

==> sections/sup.tex <==
Related work comparison

\input{tables/rel_work}


\begin{figure*}
\centering
\begin{subfigure}{0.8\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{images/survey_details.png}
  \label{fig:sfig1}
\end{subfigure}%
\caption{Possibility of privacy invasion comparing face images with masked face images}
\label{fig:utksummary}
\end{figure*}



For \cite{das2018mitigating}, we are unable to do a 1 to 1 comparison with our data split as the project link from their paper is not available on github anymore.


